The Many Qualities of a New Directly Accessible Compression Scheme

We present a new variable-length computation-friendly encoding scheme, named SFDC (Succinct Format with Direct aCcesibility), that supports direct and fast accessibility to any element of the compressed sequence and achieves compression ratios often higher than those offered by other solutions in the literature. The SFDC scheme provides a flexible and simple representation geared towards either practical efficiency or compression ratios, as required. For a text of length $n$ over an alphabet of size $\sigma$ and a fixed parameter $\lambda$, the access time of the proposed encoding is proportional to the length of the character's code-word, plus an expected $\mathcal{O}((F_{\sigma - \lambda + 3} - 3)/F_{\sigma+1})$ overhead, where $F_j$ is the $j$-th number of the Fibonacci sequence. In the overall it uses $N+\mathcal{O}\big(n \left(\lambda - (F_{\sigma+3}-3)/F_{\sigma+1}\big) \right) = N + \mathcal{O}(n)$ bits, where $N$ is the length of the encoded string. Experimental results show that the performance of our scheme is, in some respects, comparable with the performance of DACs and Wavelet Tees, which are among of the most efficient schemes. In addition our scheme is configured as a \emph{computation-friendly compression} scheme, as it counts several features that make it very effective in text processing tasks. In the string matching problem, that we take as a case study, we experimentally prove that the new scheme enables results that are up to 29 times faster than standard string-matching techniques on plain texts.

==> fig-bht-dht.tex <==
\begin{figure}[!t]
\begin{scriptsize}
    \centering
$$
\begin{array}{ll}
    & \textrm{Balanced Huffman Tree}\\[0.2cm]
    & \texttt{ a :  00 }\\
    & \texttt{ c :  01 }\\
    & \texttt{ g :  10 }\\
    & \texttt{ t :  11 }\\[0.5cm]
    \hline
    & \texttt{ \,0 1 2 3 4 5 6 7 8 9 A B C D F }\\[0.2cm]
    & \texttt{ \,t g c a t g c a t g c a t g c }\\[0.1cm]

    \begin{array}{l}
        \widehat{Y}_0 =\\
    \end{array} &
    \begin{array}{|l|}
        \hline
        \texttt{ 1 1 0 0 1 1 0 0 1 1 0 0 1 1 0 }\\
        \hline
    \end{array}\\[0.1cm]
    
    \begin{array}{l}
        \widehat{Y}_D =\\
        \end{array} &
    \begin{array}{|l|}
    \hline
        \cellcolor{black!15}\texttt{ 1 0 1 0 1 0 1 0 1 0 1 0 1 0 1 }\\
    \hline
    \end{array}\\[0.2cm]
    &~{\color{gray}\texttt{\! }}\\
\end{array}~~~~~~~~
\begin{array}{ll}
    & \textrm{Degenerate Huffman Tree}\\[0.2cm]
    & \texttt{ a :  0 }\\
    & \texttt{ c :  10 }\\
    & \texttt{ g :  110 }\\
    & \texttt{ t :  1110 }\\[0.5cm]
    \hline    
    & \texttt{ \,0 1 2 3 4 5 6 7 8 9 A B C D F }\\[0.2cm]
    & \texttt{ \,t g c a a c a a g c a a c a a }\\[0.1cm]

    \begin{array}{l}
        \widehat{Y}_0 =\\
    \end{array} &
    \begin{array}{|l|}
        \hline
        \texttt{ 1 1 1 0 0 1 0 0 1 1 0 0 1 0 0 }\\
        \hline
    \end{array}\\[0.1cm]
    
    \begin{array}{l}
        \widehat{Y}_D =\\
        \end{array} &
    \begin{array}{|l|}
    \hline
        \cellcolor{black!15}\texttt{ {\color{red}1} {\color{blue}1} {\color{Green}0} {\color{blue}0} {\color{red}1} {\color{Green}0} {\color{red}0} - {\color{blue}1} {\color{Green}0} {\color{blue}0} - {\color{Green}0} - - }\\
        %{\color{red}1} {\color{red}1} {\color{Green}0} {\color{Green}1} {\color{red}0} {\color{red}1} {\color{red}0} {\color{blue}0} {\color{blue}0} }\\
    \hline
    \end{array}\\[0.2cm]
    %{\color{red}1} {\color{red}1} {\color{green}0} {\color{green}1} {\color{red}0} {\color{red}1} {\color{red}0} {\color{blue}0} {\color{blue}0}
    
    &~{\color{gray}\texttt{\! 0 1 2 1 0 5 0 - 8 9 8 - C - - }}\\
\end{array}
$$
\end{scriptsize}
    \caption{.}
    \label{fig:bht-dht}
\end{figure}

==> fig-example-worst.tex <==
\definecolor{Green}{rgb}{0,0.8,0.5}
\begin{figure}[!t]
    \centering
% z = 100010110101
% ! = 1000101101001110
$$
\begin{array}{ll}
    & \texttt{ \,0 1 2 }\\[0.2cm]
    \hline
    & \texttt{ \,z z ! }\\

    \begin{array}{l}
        \widehat{Y}_0 =\\
    \end{array} &
    \begin{array}{|l|}
        \hline
        \texttt{ 1 1 1 }\\
        \hline
    \end{array}\\[0.1cm]
    
    \begin{array}{l}
        \widehat{Y}_1 =\\
    \end{array} &
    \begin{array}{|l|}
        \hline
        \texttt{ 0 0 0 }\\
        \hline
    \end{array}\\[0.1cm]

    \begin{array}{l}
        \widehat{Y}_2 =\\
    \end{array} &
    \begin{array}{|l|}
        \hline
        \texttt{ 0 0 0 }\\
        \hline
    \end{array}\\[0.1cm]

    \begin{array}{l}
        \widehat{Y}_3 =\\
    \end{array} &
    \begin{array}{|l|}
        \hline
        \texttt{ 0 0 0 }\\
        \hline
    \end{array}\\[0.1cm]

    \begin{array}{l}
        \widehat{Y}_4 =\\
    \end{array} &
    \begin{array}{|l|}
        \hline
        \texttt{ 1 1 1 }\\
        \hline
    \end{array}\\[0.1cm]

    \begin{array}{l}
        \widehat{Y}_D =\\
        \end{array} &
    \begin{array}{|l|}
    \hline
        \cellcolor{black!15}\texttt{ {\color{blue}0} {\color{Green}0} 
        {\color{red}0} {\color{red}1} {\color{red}1} {\color{red}0} {\color{red}1} {\color{red}0} {\color{red}0} {\color{red}1} {\color{red}1} {\color{red}1} {\color{red}0} 
        {\color{Green}1} {\color{Green}1} {\color{Green}0} {\color{Green}1} {\color{Green}0} {\color{Green}1}
        {\color{blue}1} {\color{blue}1} {\color{blue}0} {\color{blue}1} {\color{blue}0} {\color{blue}1}
        }\\
    \hline
    \end{array}\\[0.2cm]
    %{\color{red}1} {\color{red}1} {\color{green}0} {\color{green}1} {\color{red}0} {\color{red}1} {\color{red}0} {\color{blue}0} {\color{blue}0}
    
    &~{\color{gray}\texttt{\! 0 1 2 2 2 2 2 2 2 2 2 2 2 1 1 1 1 1 1 0 0 0 0 0 0 }}
\end{array}
$$
    \caption{The \newenc representation of the string \texttt{zz!} with $5$ fixed layers. The fixed layers have a white background, while the dynamic layer has a grey one. The pending bits have been arranged linearly along the dynamic layer according to a last-in first-out approach.
    }
    \label{fig:ex-worst}
\end{figure}

==> fig-huffman-tree.tex <==
\begin{figure}[!t]
  \begin{center}
    \begin{footnotesize}
    \begin{tabular}{|c|}
    \hline
      \begin{tabular}{ll}
        \texttt{t} :& \texttt{00}\\
        \texttt{e} :& \texttt{01}\\
        \texttt{w} :& \texttt{100}\\
        \texttt{a} :& \texttt{101}\\
        \texttt{n} :& \texttt{110}\\
        \texttt{y} :& \texttt{1110}\\
        \texttt{b} :& \texttt{1111}\\
      \end{tabular}
      \begin{tabular}{l}
        \includegraphics[width=0.44\textwidth]{tree2}\\
      \end{tabular}
      \begin{tabular}{ll}
        \texttt{twenty} ~~~~& \texttt{\={0}0\={1}00\={0}1\={1}10\={0}0\={1}110}\\
        \texttt{ten}    & \texttt{\ \ \ \={0}0\={0}1\={1}10}\\
        \texttt{ten}    & \texttt{\ \ \ \ \ \ \ \ \ \={0}0\={0}1\={1}10}\\
      \end{tabular}\\
    \hline
    \end{tabular}
    \end{footnotesize}
    \caption{A Huffman code for the set of symbols
      $\{$\texttt{t}, \texttt{e}, \texttt{w}, \texttt{a}, \texttt{n},
      \texttt{y}, \texttt{b}$\}$. The binary string
      \texttt{\={0}0\={1}00\={0}1\={1}10\={0}0\={1}110} is the
      encoding of the string \texttt{twenty}, where a ``bar'' indicates
      the starting bit of each codeword. Two occurrences of the binary
      string \texttt{ten} start at the $4$-th and $10$-th bit of the
      encoded version of the string \texttt{twenty}. However, each of them is a false match.}
    \label{fig:huffman-tree}
  \end{center}
\end{figure}

==> survey.tex <==


%In this section we briefly review the main known solutions for direct accessing a text coded by a variable-length encoding.

Let $y$ be a text of length $n$ over an alphabet of size $\sigma$, and let $N_{0} \defAs n \cdot \lceil \log \sigma \rceil$ be the number of bits in the minimal fixed-length representation of $y$. Also, let $Y \defAs \rho(y[0])\rho(y[1]) \cdots \rho(y[n-1])$ be an encoding of $y$ by a variable-length code $\rho$, and let $N \defAs \sum_{i=0}^{n-1} |\rho(y[i])|$ be the bit-length of $y$.
%In this section we briefly review the main known solutions for direct accessing a sequence of $n$ variable-length codes, i.e. to the problem of efficiently extracting (not necessarily in constant time) the $i$-th character of the original text $y$, for $0\leq i < n$. As before, let $N$ be the length in bits of the coded, i.e. $N=\sum_{i=0}^{n-1}|\rho(y[i])|$. In addition, let $N_0 = \sum_{i=0}^{n-1} (\lfloor \log([y[i]]) \rfloor+1)$ be the total length of the representation if we could assign just the minimum number of bits required to represent each symbol of the text. We indicate with symbol $M$ maximum value in $\Sigma$.


\begin{table}[!t]
    \centering
    \begin{tabular}{|l|l|l|}
        \hline
        &&\\[-0.3cm]
         Method & Reference & Additional Space\\
        &&\\[-0.3cm]
        \hline
        &&\\[-0.3cm]
        Sparse Sampling & - & $\lceil n/h\rceil \lceil \log(N)\rceil$\\
        &&\\[-0.3cm]
        Dense Sampling & \cite{FV07} & $n(\log \log N + \log \log M)$\\
        &&\\[-0.3cm]
        Elias-Fano  & \cite{Elias74} & $N_0 + n \log(N_0/n) + \mathcal{O}(n)$ \\
        &&\\[-0.3cm]
        Interpolative Coding  & \cite{MoffatS00,Teuhola11} & $\mathcal{O}(n \log(N)/ \log(n))$ \\
        &&\\[-0.3cm]
        Wavelet Tree & \cite{GGV03} & $N + o(N)$\\
        &&\\[-0.3cm]
        Directly Addressable Codes & \cite{BLN09a,BLN13} & $\mathcal{O}(\frac{N\log \log N}{b \log N} + \log M)$\\
        Succinct Format Direct Accessibility & This paper~~~ & $N+O(n)$\\
        \hline
    \end{tabular}\\[0.4cm]
    \caption{\color{red}Caption}
    \label{tab:my_label}
\end{table}


The most classical solution is the \emph{sparse sampling} method,  based on sampling the encoded sequence. Having fixed an integer parameter $h>1$ upon which the sampling density depends, the initial position of the encoding of every $h$-th element of the text is maintained in an auxiliary vector. Access to the $(\nu h + d)$-th position, where $0\leq d < h$, is done by decoding the $d$ characters starting from  position $\nu h$. This results in a space overhead of $\lceil n/h\rceil \lceil \log N\rceil$ bits and a time overhead of $\mathcal{O}(h)$ to directly access any element, assuming one can decode each symbol in constant time.

An improvement in this direction is represented by \emph{dense sampling} \cite{FV07}. This technique represents the $i$-th character of the text using only $\log(y[i])$ bits and uses two levels of pointers to characters in the text: a first level of pointers to absolute positions, one every $\Theta(\log N)$ characters in the text; and a second level of relative pointers, for the remaining characters in the text. This allows access to each character in constant time using an extra space equal to $O(n(\log \log N + \log \log \sigma))$.
%, where $M$ is the largest number in the sequence.

The \emph{Elias-Fano-based representation} \cite{Elias74} is designed to compress a sequence $y$ of $n$ strictly increasing number values. Such a representation separates the $s=\lceil \log(y_{n-1}/n)\rceil$ lower bits of each element from the remaining upper bits and stores the lower bits contiguously within an array. The upper bits are instead represented in another array of bits of size at most $2n$, in which the bits at positions $\lceil y_i/2s \rceil + i$ are set, for $0\leq i < n$. 
The Elias-Fano representation thus uses a space equal to $n \log(y_{n-1}/n) + \mathcal{O}(n)$. In addition, using more recent techniques to find the $i$-th bit set in a bitmap in constant time and extra space $o(n)$ \cite{???}, any symbol in the sequence can be retrieved in constant time.

Finally, we observe that this representation can be used to encode a generic sequence $y$ of $n$ symbols (interpreted as positive integers) by concatenating the binary representations of the numeric values $y_i + 1$, excluding their most significant bit set, into a new sequence. The initial positions of the encoded numbers in this new sequence are strictly increasing and can therefore be stored using the Elias-Fano representation described above. Overall, the technique achieves a constant access time using a space of $N_0 + n \log(N_0/n) + \mathcal{O}(n)$ bits.

The \emph{Interpolative Coding} \cite{MoffatS00,Teuhola11} is a technique for encoding sequences of integers using variable-length codes, so as to allow fast access both to the symbol having a given position and to the symbol for which the sum of the symbols preceding it exceeds a certain threshold. Both operations are supported in $\mathcal{O}(\log n)$ time. The idea is to create a balanced virtual tree on the sequence of the encoded values. The encoding of a subtree is preceded by the sum of the values and the encoding size of the left subtree. The space overhead is only $\mathcal{O}(n \log N/ \log n)$ bits. This solution offers a good combination of space and time efficiency for both operations, but does not perform well from a practical point of view when compared to the other solutions. 

The \emph{Wavelet Tree} \cite{GGV03} by Grossi \emph{et al.} is a data structure that can be used for the representation of a sequence of $n$ symbols encoded with variable-length encoding and allowing direct access in time proportional to the length of the encoding. The root of the wavelet tree is a bitmap containing the first bits of all codewords $\rho(y_i)$, for $0\leq i<n$. If there are some bits equal to $0$ in this bitmap, then the left child of the node contains the next bit of the codewords that begin with a bit set to $0$. Similarly, if there are some bits set to $1$ in the bitmap, then the right child of the node contains the second bit of those codewords that begin with a bit set to $1$. The operation continues recursively on both children. The total number of bits in the wavelet tree is exactly $N$ and the wavelet tree replaces the encoded sequence. The decoding of a character $y_i$ can be performed by following the bits on the nodes of the tree, starting at the root, and descending left or right based on the bit value read at each node. Each time one descends on a child node, the new position is computed using the function \textsc{rank}$(B,b)$ which returns the number of occurrences of bit $b$ in a bitmap $B$. Since this function can be computed in constant time using only $o(n)$ additional bits with respect to B \cite{???}, each character $y[i]$ can be accessed in $\mathcal{O}(|\rho(y[i])|))$. The total space used for the data structure is $N + o(N)$ bits, plus the pointers to the tree structure.

The \emph{Directly Addressable Codes} (DACs) \cite{BLN09a,BLN13} make use of the generalized Vbyte coding \cite{Williams1999}. The symbols are first encoded into a sequence of $(b + 1)$-bit chunks. The representation uses several bitstreams to arrange the chuncks of the codewords. The first bitstream contains the least significant chunk of every codeword, the second one contains the second chunk of every codeword, and so on. Thus $\lceil \log(M)/b \rceil$ bitstreams are needed.
Each bitstream  is separated into two parts. The lowest $b$ bits of the chunks will be stored contiguously in an array $A$, whereas the highest bits will be concatenated into a bitmap $B$. 
The bits in $B$ identify whether there is a chunk of that codeword in the next bitstream. To find the position of the corresponding chunk in the next bitstream, a rank queries data structure is needed on the bitmap $B$.
The overall space is essentially that of the Vbyte representation of the sequence, plus (significantly) lower-order terms, and specifically $\mathcal{O}(\log M)$ space for the pointers and $\mathcal{O}(\frac{N\log \log N}{b \log N})$ for the rank data structure.

To decode the $i$-th symbol of the sequence, one can collect the chunks by moving from the first to the last bitstream until the corresponding bit in the array B is set to zero. 
Therefore, the expected number of accesses required for the extraction of a symbol is $\lceil N/(n(b + 1))\rceil$, while the worst case requires $\lceil \log(M)/b\rceil$ accesses. 




==> tab-huffman-codes.tex <==
\begin{table}[!t]
\centering
\begin{scriptsize}
\begin{tabular*}{0.85\textwidth}{@{\extracolsep{\fill}}cclc}
\textbf{rank} & \textbf{char} & \textbf{code} & \textbf{ length}\\
\hline
1 & \virg{space} & \texttt{00} & 2 \\
2 & \virg{e} & \texttt{010} & 3 \\
3 & \virg{a} & \texttt{1011} & 4 \\
6 & \virg{n} & \texttt{0111} & 4 \\
7 & \virg{o} & \texttt{11111} & 5 \\
8 & \virg{d} & \texttt{11101} & 5 \\
8 & \virg{s} & \texttt{11100} & 5 \\
10 & \virg{i} & \texttt{11010} & 5 \\
15 & \virg{,} & \texttt{110000} & 6 \\
18 & \virg{y} & \texttt{011010} & 6 \\
19 & \virg{b} & \texttt{1111010} & 7 \\
20 & \virg{c} & \texttt{1111001} & 7 \\
21 & \virg{g} & \texttt{1111000} & 7 \\
22 & \virg{A} & \texttt{1100010} & 7 \\
37 & \virg{E} & \texttt{1100011010} & 10 \\
51 & \virg{z} & \texttt{100010110101} & 12 \\
60 & \virg{!} & \texttt{1000101101001110} & 16 \\
\end{tabular*}\\[0.2cm]
\end{scriptsize}
\caption{Prefix codes of some characters of the alphabet relative to the natural language text analysed in Fig.~\ref{fig:huffman-code-length}}
\label{tab:hoffman-codes}
\end{table}

